SmartFL: Semantics Based Probabilistic Fault Localization

Testing-based fault localization has been a research focus in software engineering in the past decades. It localizes faulty program elements based on a set of passing and failing test executions. Since whether a fault could be triggered and detected by a test is related to program semantics, it is crucial to model program semantics in fault localization approaches. Existing approaches either consider the full semantics of the program (e.g., mutation-based fault localization and angelic debugging), leading to scalability issues, or ignore the semantics of the program (e.g., spectrum-based fault localization), leading to imprecise localization results. Our key idea is: by modeling only the correctness of program values but not their full semantics, a balance could be reached between effectiveness and scalability. To realize this idea, we introduce a probabilistic model by efficient approximation of program semantics and several techniques to address scalability challenges. Our approach, SmartFL(SeMantics bAsed pRobabilisTic Fault Localization), is evaluated on a real-world dataset, Defects4J 2.0. The top-1 statement-level accuracy of our approach is {14\%}, which improves 130\% over the best SBFL and MBFL methods. The average time cost is {205} seconds per fault, which is half of SBFL methods. After combining our approach with existing approaches using the CombineFL framework, the performance of the combined approach is significantly boosted by an average of 10\% on top-1, top-3, and top-5 accuracy compared to state-of-the-art combination methods.

==> macros.tex <==
\usepackage{xspace}

\usepackage[english]{babel}
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

% \newcommand{\citet}[1]{\cite{#1}}

\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\todo}[1]{{\color{red} \bf \{TODO: {#1}\}}}
\newcommand{\thename}{{SmartFL}\xspace}
% \newcommand{\thename}{{SmartFL-v0}\xspace}
\newcommand{\thenamedetail}{{\textbf{S}e\textbf{M}antics b\textbf{A}sed p\textbf{R}obabilis\textbf{T}ic \textbf{F}ault \textbf{L}ocalization}}
%\newcommand{\repo}{{https://doi.org/10.5281/zenodo.5440090}}
\newcommand{\repo}{\textbf{\url{https://github.com/toledosakasa/SMARTFL}}}


\def\modify#1#2#3{{\small\underline{\sf{#1}}:} {\color{red}{\small #2}}
{{\color{red}\mbox{$\Rightarrow$}}} {\color{blue}{#3}}}
%\renewcommand{\modify}[3]{{#3}}

\newcommand{\yxmodify}[2]{\modify{Yingfei}{#1}{#2}}
\newcommand\mymargin[1]{\marginpar{{\flushleft\textsc\footnotesize {#1}}}}
\newcommand\yxmargin[1]{\mymargin{YX:\;#1}}

\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\eqnref}[1]{violation~\eqref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\tblref}[1]{Table~\ref{#1}}
\newcommand{\theref}[1]{Theorem~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\smalltitle}[1]{{\smallskip \noindent \bf  {#1}.\ }}
\newcommand{\smalltitlecolon}[1]{{\smallskip \noindent \bf  {#1}:\ }}

\newtheorem{property}{Property}

\newcommand{\yxmodifyok}[2]{#2}

\newcommand{\mycomment}[2]{{\small\color{magenta}\underline{\sf{#1}}:} {\color{magenta}{\small #2}}}
\newcommand{\yxcomment}[1]{\mycomment{Yingfei}{#1}}

\newcommand{\mycommentblue}[2]{{\small\color{blue}\underline{\sf{#1}}:} {\color{blue}{\small #2}}}
\newcommand{\zmhcomment}[1]{\mycommentblue{Zmh}{#1}}

\newcommand{\hdcomment}[2]{\mycomment{Dan}{#2}}
\newcommand{\lxycomment}[1]{\mycomment{Xinyuan}{#1}}

\newcommand{\xzcomment}[1]{\mycomment{Xin}{#1}}

% \newcommand{\wyqmodify}[2]{{\color{red} {#1} $\Rightarrow$} {\color{blue} {#2}}}
\newcommand{\wyqmodify}[2]{{#1}}

\usepackage{listings}

\usepackage{hyperref}

\definecolor{boxgray1}{rgb}{0.95,0.95,0.95}
\usepackage[most]{tcolorbox}
\newtcbtheorem{Summary}{\bfseries Summary}{enhanced,drop shadow={black!50!white},
  coltitle=black,
  top=0.1in,
  attach boxed title to top left=
  {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=boxgray1}
}{summary}
% \newtcolorbox[auto counter]{summary}[1][]{title={\bfseries Summary~\thetcbcounter},enhanced,drop shadow={black!50!white},
%   coltitle=black,
%   top=0.3in,
%   attach boxed title to top left=
%   {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
%   boxed title style={size=small,colback=white},#1}


% \renewcommand{\yxcomment}[1]{}
% \renewcommand{\yxmodify}[2]{#2}

% \newtoggle{longversion}
% % \toggletrue{longversion}
% \togglefalse{longversion}

% \newtoggle{patchtype}
% % \toggletrue{patchtype}
% \togglefalse{patchtype}

